Identifying partial mouse brain microscopy images from Allen reference atlas using a contrastively learned semantic space

Precise identification of mouse brain microscopy images is a crucial first step when anatomical structures in the mouse brain are to be registered to a reference atlas. Practitioners usually rely on manual comparison of images or tools that assume the presence of complete images. This work explores Siamese Networks as the method for finding corresponding 2D reference atlas plates for given partial 2D mouse brain images. Siamese networks are a class of convolutional neural networks (CNNs) that use weight-shared paths to obtain low dimensional embeddings of pairs of input images. The correspondence between the partial mouse brain image and reference atlas plate is determined based on the distance between low dimensional embeddings of brain slices and atlas plates that are obtained from Siamese networks using contrastive learning. Experiments showed that Siamese CNNs can precisely identify brain slices using the Allen mouse brain atlas when training and testing images come from the same source. They achieved TOP-1 and TOP-5 accuracy of 25% and 100%, respectively, taking only 7.2 seconds to identify 29 images.

==> chapters/conclusions.tex <==
\vspace{-0.25cm}
\section{Conclusions}
\vspace{-0.25cm}
In this study, we proposed Siamese Networks as a method for identifying complete and partial mouse brain slices, i.e. finding the corresponding 2D atlas plates. The networks have shown a high precision and significantly improved inference time compared to the baseline. While we demonstrated this with a 2D reference atlas, the same method can also be applied to a 3D reference atlas for even higher identification precision.

==> chapters/discussions.tex <==
%\vspace{-0.25cm}
\section{Discussions \& Conclusions}
%\vspace{-0.25cm}
 The Siamese networks used to identify brain slices has shown impressive results, i.e. in finding corresponding coronal 2D atlas plates. It achieved TOP-5 accuracy of 100\% meaning that the actual corresponding atlas plate always falls in the top 5 predicted atlas plates. The identification accuracy (MAE) had no clear correlation with the batch size (16 and 32), the image resolution ($224\times224$, $448\times448$, $1024\times1024$) and the type of the base for the Siamese network (ResNet50v2 and ResNet101v2). However, using images with lower resolution and networks with fewer parameters could improve the inference time.  We did not observe that the performance of the Siamese network would be highly influenced by the loss function, namely contrastive and triplet losses. The models trained with triplet loss rather than contrastive loss, on average, achieved higher accuracy, however, the difference is not significant. 
 
 The Siamese networks produced impressive results even though some images of different classes looked very similar to each other, thus making the identification task even more complex. The distance between such images should be lower than the distance between two completely dissimilar images. Maximizing the distance between all images of different classes would make it difficult for networks to learn representations of these classes. Contrastive and triplet losses solve this issue by using margin, i.e., dissimilar images are not pushed away if the distance between them is larger than the margin.
 

 In this study, we proposed Siamese Networks as a method for identifying complete and partial mouse brain slices, i.e. finding the corresponding 2D atlas plates. The networks have shown a high precision and significantly improved inference time compared to the baseline. While we demonstrated this with a 2D reference atlas, the same method can also be applied to a 3D reference atlas for even higher identification precision.

